Computable convergence rate bound for ratio consensus algorithms

The objective of the paper is to establish a computable upper bound for the almost sure convergence rate for a class of ratio consensus algorithms defined via column-stochastic matrices. Our result extends the works of Iutzeler et al. (2013) on similar bounds that have been obtained in a more restrictive setup with limited conclusions. The present paper complements the results of Gerencs\'er and Gerencs\'er (2021), identifying the exact almost sure convergence rate of a wide class of ratio consensus algorithms in terms of a spectral gap, which is, however, not computable in general. The upper bound provided in the paper will be compared to the actual rate of almost sure convergence experimentally on a range of modulated random geographic graphs with random local interactions.

==> decl_IEEE.tex <==
\bibliographystyle{plain}


%%%%%%%%% various packages %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{hyperref}
\usepackage{amssymb,amsmath}
\usepackage{amsfonts}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage{fancyhdr}
\usepackage{yfonts}
\usepackage{mathrsfs}
\usepackage[dvips]{graphicx}
\usepackage{enumerate}
\usepackage{xspace}
%\usepackage[rflt]{floatflt}
\usepackage{cite}
%\usepackage{amsthm}

%\usepackage{algorithm}
%\floatname{algorithm}{Alg.}
%\usepackage{algorithmic}
\usepackage{psfrag}
\usepackage{url}


%%%%%%%%% Commenting commands %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand{\margincom}[1]{\marginpar{{\small#1}}}

\usepackage[dvipsnames]{xcolor}
\usepackage{xcolor}
\usepackage{lipsum}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\YellowOrange}[1]{\textcolor{YellowOrange}{#1}}
\usepackage{verbatim}

\newcommand{\sam}[1]{\blue{#1}}
\providecommand{\comsam[1]}{\sam{\com{SAM}{#1}}}
\newcommand{\jh}[1]{{#1}}

\providecommand{\comjh[1]}{\jh{\textcolor{blue}{\com{JH}{#1}}}}
\providecommand{\com[2]}{\begin{tt}[#1: #2]\end{tt}}
\usepackage{color}
\newcommand{\JMH}[1]{#1}
\newcommand{\modif}[1]{{\color{blue}#1}}
\newcommand{\jnt}[1]{{#1}}

%%%%%%%%%%%% "Theorems" %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{requirement}[theorem]{Requirement}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{problem}[theorem]{Problem}
%\newtheorem{proof}{Proof}
%\graphicspath{{figures_recentes/}}


\providecommand{\sol[1]}{\vspace{.5cm}\noindent {\textbf{Solution de l'exercice #1}}\\}


%%%%%%%%%%%%% Mathematical macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand{\prt}[1]{\left( #1 \right)}
\providecommand{\C}{\mathbb{C}} 
\providecommand{\PP}{\mathbb{P}}
\providecommand{\e}{\phantom{aaa}}
\providecommand{\abs[1]}{\left|#1\right|}
\providecommand{\norm[1]}{\abs{\abs{#1}}}%
\providecommand{\floor[1]}{\lfloor  #1 \rfloor }
\providecommand{\ceil[1]}{\lceil #1  \rceil}
\providecommand{\1}{\textbf{1}}
\providecommand{\0}{\textbf{0}}\providecommand{\quotes[1]}{``#1"}
\providecommand{\scalprod[2]}{\left<#1,#2\right>}%
\providecommand{\Linf}{{\mathcal{L}_\infty}}
\providecommand{\sign}[1]{\mathrm{sign}\prt{#1}}

\providecommand{\L}{{\mathcal{L}}}



\providecommand{\matr[4]}{\left(\begin{array}{cc}#1 & #2 \\ #3
&#4\end{array}\right) }
\providecommand{\hvec[2]}{\left(\begin{array}{cc}#1 &
#2\end{array}\right) }
\providecommand{\vvec[2]}{\left(\begin{array}{c}#1 \\
#2\end{array}\right) }




\def\0{{\bf 0}}
\def\R{\mathbb{R}}
\def\N{\mathbb{N}}
\def\Z{\mathbb{Z}}
\def\Q{\mathbb{Q}}
\def\I{{\bf I}}
 \def\V{\mathcal{V}}
 \def\M{\mathcal{M}}
  \def\S{\mathcal{S}}
 \def\U{\mathcal{U}}
 \def\C{\mathcal{C}}
\def\G{\mathcal{G}}
\def\T{\mathcal{T}}
\def\EE{\mathcal{E}}
\def\E{\mathbb{E}}
\def\DD{\mathcal{D}}
\def\NN{\mathcal{N}}
\newcommand{\unn}{\{1,\ldots, n\}}
\newcommand{\ie}{{\it i.e. }}
\newcommand\TODO[1]{\textbf{TODO: \textit{#1}}}

\newcommand{\ssum}{\displaystyle\sum}
\newcommand{\Var}[1]{\text{Var}{#1}}

\newcommand{\rpm}{\raisebox{.2ex}{$\scriptstyle\pm$}}
\newcommand{\ooneovern}{o\left(\frac{1}{n}\right)}


\providecommand{\RR}{\mathbb{R}}
